Ca2-VDM: Efficient Autoregressive Video Diffusion Model with Causal Generation and Cache Sharing

With the advance of diffusion models, today's video generation has achieved impressive quality. To extend the generation length and facilitate real-world applications, a majority of video diffusion models (VDMs) generate videos in an autoregressive manner, i.e., generating subsequent clips conditioned on the last frame(s) of the previous clip. However, existing autoregressive VDMs are highly inefficient and redundant: The model must re-compute all the conditional frames that are overlapped between adjacent clips. This issue is exacerbated when the conditional frames are extended autoregressively to provide the model with long-term context. In such cases, the computational demands increase significantly (i.e., with a quadratic complexity w.r.t. the autoregression step). In this paper, we propose Ca2-VDM, an efficient autoregressive VDM with Causal generation and Cache sharing. For causal generation, it introduces unidirectional feature computation, which ensures that the cache of conditional frames can be precomputed in previous autoregression steps and reused in every subsequent step, eliminating redundant computations. For cache sharing, it shares the cache across all denoising steps to avoid the huge cache storage cost. Extensive experiments demonstrated that our Ca2-VDM achieves state-of-the-art quantitative and qualitative video generation results and significantly improves the generation speed. Code is available: https://github.com/Dawn-LX/CausalCache-VDM

==> Tables/2_fintune_on_ucf101.tex <==
\begin{table}[!h]
    \addtolength{\tabcolsep}{-2.5pt}
     \caption{Finetuned FVD scores on UCF-101 test set. $^*$ means trained on both train and test sets.}
    \centering
    \small
       \begin{tabular}{lcc}
        \hline
        Method & Res. & FVD    \\ \hline
        MCVD~\cite{Voleti2022MCVD}    & $64^2$   & 1143   \\
        VDT~\cite{lu2024vdt}     & $64^2$   & 225.7  \\ \hline
        DIGAN$^*$~\cite{yu2022generating}   & $128^2$ & 577    \\
        % DIGAN   & $128^2$ & 655    \\
        TATS~\cite{ge2022long}    & $128^2$ & 420    \\ 
        VideoFusion~\cite{luo2023videofusion}   & $128^2$ & 220    \\ \hline
        LVDM$^*$~\cite{he2022latent}    & $256^2$ & 372    \\
        PVDM~\cite{yu2023video}    & $256^2$ & 343.6  \\
        Latte~\cite{ma2024latte}   & $256^2$ & 333.6 \\
        Causal-VDM    & $256^2$ & \textbf{184.5} \\ \hline
        \end{tabular}
       % \vspace{-0.5em}
       \label{tab:finetune}
\end{table}

